Systematic NICER study of the low-ionized Fe K$\alpha$ line on RS Canum Venaticorum type stars

The Fe K$\alpha$ fluorescence line ($\sim 6.4$ keV) has been observed during solar and stellar flares. Two emission mechanisms of the Fe K$\alpha$ line, photoionization and collisional ionization, have been discussed, and the aim of this work is to collect evidences for each mechanism employing a statistical correlation approach between the Fe K$\alpha$ line flux and rough flare properties. Here, we systematically searched the NICER (0.2$-$12 keV) archive data for the Fe K$\alpha$ line of RS Canum Venaticorum type stars. Among our analyzed 255 observation IDs with a total exposure of $\sim 700$ ks, we found 25 data sets (total $\sim 40$ ks) exhibiting the Fe K$\alpha$ emission line at 6.37$-$6.54 keV with its equivalent width of 44.3$-$578.4 eV: 18 observations during flares, 6 observations during unconfirmed possible flare candidates and one at a quiescent phase. These observations indicate a positive correlation between the Fe K$\alpha$ line intensity and the 7.11$-$20 keV thermal plasma luminosity with its powerlaw index of $0.86 \pm 0.46$. This correlation in the range of the thermal plasma luminosity $10^{29-33}$ erg s$^{-1}$ is consistent with the photoionization origin of the line. On the other hand, the equivalent width of the Fe K$\alpha$ line has a negative correlation with the 7.11$-$20 keV thermal plasma luminosity with its powerlaw index of $-0.27 \pm 0.10$. This anti-correlation is consistent with the decline of the fluorescence efficiency with increasing the stellar flare loop height. Furthermore, we found a signature of an absorption line at $6.38^{+0.03}_{-0.04}$ keV during a superflare of $\sigma$ Gem. The equivalent width of the line was $-34.7^{+2.03}_{-1.58}$ eV. We discuss the density of the Fe ions from the equivalent width using the curve of growth analysis.

==> table/GT_Mus/1100140102_block5.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:GTMus_G1_app}b \& c.}
\begin{center}
\begin{tabular}{cccccc}
\hline
\multicolumn{6}{c}{1100140102 GTI 5 (During Flare G1 on GT Mus)}                                                                    \\ \hline
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline 
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$4.08^{+1.92}_{-1.49}$ / $47.3^{+22.3}_{-17.3}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $4.11^{+2.37}_{-1.64}$ /  $47.7^{+27.5}_{-19.0}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.27^{+0.12}_{-0.11}$} &                                   & $Z$ ($Z_{\odot}$) & $0.26^{+0.14}_{-0.11}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.33^{+0.33}_{-0.11}$} &                                   & $K^{\mathrm{apec}}$ & $0.32^{+0.39}_{-0.10}$    \\ \cline{4-6} 
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.49^{+0.09}_{-0.08}$ \\  
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\ 
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $3.58^{+0.60}_{-0.12}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{20 (29)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 14 (27) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.89} & \multicolumn{2}{c}{Null hyp. prob.} &   0.98  \\ \hline
\end{tabular}
\end{center}
\label{tab:1100140102_block5}
\end{table*}

==> table/GT_Mus/1100140108_block_all.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:GTMus_Quiescent}b \& c.}
\begin{center}
\begin{tabular}{cccccc}
\hline
\multicolumn{6}{c}{1100140108 All (During quiescent phase on GT Mus)}  \\ \hline
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$3.23^{+1.22}_{-1.04}$ / $37.5^{+14.2}_{-12.0}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $2.74^{+1.29}_{-0.75}$ /  $31.8^{+15.0}_{-8.7}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.18^{+0.06}_{-0.06}$} &                                   & $Z$ ($Z_{\odot}$) & $0.18^{+0.06}_{-0.06}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.06^{+0.06}_{-0.02}$} &                                   & $K^{\mathrm{apec}}$ & $0.08^{+0.07}_{-0.03}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.44^{+0.07}_{-0.06}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $0.28^{+0.19}_{-0.18}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{36 (29)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 30 (27) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.17} & \multicolumn{2}{c}{Null hyp. prob.} &   0.31  \\ \hline
\end{tabular}
\end{center}
\label{tab:1100140108_block_all}
\end{table*}


==> table/HD251108/5203530103_block_all.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:HD251108_H1}b \& c.}
\begin{center}
\begin{tabular}{cccccc}
\hline
\multicolumn{6}{c}{5203530103 All (During Flare HD1 on HD 251108)} \\ \hline
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$5.41^{+1.75}_{-1.71}$ / $62.7^{+20.3}_{-19.9}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $4.91^{+1.9}_{-1.51}$ /  $57.0^{+22.1}_{-17.5}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.12^{+0.07}_{-0.06}$} &                                   & $Z$ ($Z_{\odot}$) & $0.11^{+0.06}_{-0.06}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.07^{+0.04}_{-0.01}$} &                                   & $K^{\mathrm{apec}}$ & $0.07^{+0.04}_{-0.02}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.46^{+0.06}_{-0.08}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $0.36^{+0.34}_{0.26}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{47 (40)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 43 (38) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.20} & \multicolumn{2}{c}{Null hyp. prob.} &   0.27  \\ \hline
\end{tabular}
\end{center}
\label{tab:5203530103_block_all}
\end{table*}


==> table/HR1099/1114010117_block5.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:HR1099_HR1}b \& c.}
\begin{center}
\begin{tabular}{cccccc}
\hline 
\multicolumn{6}{c}{1114010117 GTI 5 (During Flare HR1 on HR 1099)}  \\ \hline 
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$4.21^{+7.45}_{-2.14}$ / $48.9^{+86.4}_{-24.9}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $3.25^{+9.49}_{-1.45}$ /  $37.7^{+110.1}_{-16.8}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.17^{+0.4}_{-0.14}$} &                                   & $Z$ ($Z_{\odot}$) & $0.14^{+0.42}_{-0.14}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.06^{+0.14}_{-0.03}$} &                                   & $K^{\mathrm{apec}}$ & $0.06^{+0.21}_{-0.03}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.48^{+0.12}_{-0.12}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $0.80^{+0.78}_{-0.78}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{18 (19)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 15 (17) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.55} & \multicolumn{2}{c}{Null hyp. prob.} &   0.61  \\ \hline 
\end{tabular}
\end{center}
\label{tab:1114010117_block5}
\end{table*}


==> table/HR1099/1114010120_block7.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:HR1099_HR2}b \& c.}
\begin{center}
\begin{tabular}{cccccc}
\hline 
\multicolumn{6}{c}{1114010120 GTI 7 (During Flare HR2 on HR 1099)}  \\ \hline 
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$3.33^{+0.52}_{-0.6}$ / $38.6^{+6.0}_{-6.9}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $3.17^{+0.55}_{-0.55}$ /  $36.8^{+6.4}_{-6.4}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.17^{+0.04}_{-0.04}$} &                                   & $Z$ ($Z_{\odot}$) & $0.17^{+0.04}_{-0.04}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.52^{+0.2}_{-0.1}$} &                                   & $K^{\mathrm{apec}}$ & $0.55^{+0.22}_{-0.12}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.39^{+0.06}_{-0.06}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $1.13^{+0.94}_{-0.94}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{37 (44)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 33 (42) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.77} & \multicolumn{2}{c}{Null hyp. prob.} &   0.84  \\ \hline 
\end{tabular}
\end{center}
\label{tab:1114010120_block7}
\end{table*}


==> table/HR1099/1114010121_block5.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:HR1099_HR2}d \& e.}
\begin{center}
\begin{tabular}{cccccc}
\hline 
\multicolumn{6}{c}{1114010121 GTI 5 (During Flare HR2 on HR 1099)}  \\ \hline 
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$3.05^{+0.8}_{-0.51}$ / $35.4^{+9.2}_{-5.9}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $2.93^{+0.76}_{-0.54}$ /  $34.0^{+8.9}_{-6.3}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.2^{+0.05}_{-0.04}$} &                                   & $Z$ ($Z_{\odot}$) & $0.2^{+0.05}_{-0.05}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.26^{+0.1}_{-0.08}$} &                                   & $K^{\mathrm{apec}}$ & $0.27^{+0.13}_{-0.08}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.40^{+0.07}_{-0.08}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $0.72^{+0.51}_{-0.52}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{49 (40)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 44 (38) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.16} & \multicolumn{2}{c}{Null hyp. prob.} &   0.25  \\ \hline 
\end{tabular}
\end{center}
\label{tab:1114010121_block5}
\end{table*}


==> table/HR1099/1114010122_block1011.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:HR1099_HR1}f \& g.}
\begin{center}
\begin{tabular}{cccccc}
\hline 
\multicolumn{6}{c}{1114010122 GTI 10+11 (During Flare HR2 on HR 1099)}  \\ \hline 
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$3.08^{+0.59}_{-0.44}$ / $35.7^{+6.8}_{-5.2}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $3.02^{+0.51}_{-0.53}$ /  $35.1^{+6.0}_{-6.1}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.19^{+0.04}_{-0.04}$} &                                   & $Z$ ($Z_{\odot}$) & $0.19^{+0.04}_{-0.04}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.22^{+0.07}_{-0.05}$} &                                   & $K^{\mathrm{apec}}$ & $0.23^{+0.09}_{-0.05}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.40^{+0.05}_{-0.04}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $0.52^{+0.35}_{-0.34}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{48 (38)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 42 (36) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.13} & \multicolumn{2}{c}{Null hyp. prob.} &   0.23  \\ \hline 
\end{tabular}
\end{center}
\label{tab:1114010122_block1011}
\end{table*}


==> table/HR1099/1114010123_block123.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:HR1099_HR2}h \& i.}
\begin{center}
\begin{tabular}{cccccc}
\hline 
\multicolumn{6}{c}{1114010123 GTI 1+2+3 (During Flare HR2 on HR 1099)}  \\ \hline 
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$2.25^{+0.37}_{-0.38}$ / $26.1^{+4.3}_{-4.4}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $2.18^{+0.41}_{-0.34}$ /  $25.3^{+4.7}_{-4.0}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.18^{+0.04}_{-0.04}$} &                                   & $Z$ ($Z_{\odot}$) & $0.17^{+0.04}_{-0.05}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.26^{+0.14}_{-0.07}$} &                                   & $K^{\mathrm{apec}}$ & $0.27^{+0.14}_{-0.08}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.49^{+0.07}_{-0.06}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $0.51^{+0.29}_{-0.27}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{38 (39)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 29 (37) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.52} & \multicolumn{2}{c}{Null hyp. prob.} &   0.83  \\ \hline 
\end{tabular}
\end{center}
\label{tab:1114010123_block123}
\end{table*}


==> table/HR1099/1114010127_block_all.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:HR1099_HR3}b \& c.}
\begin{center}
\begin{tabular}{cccccc}
\hline 
\multicolumn{6}{c}{1114010127 GTI all (During Flare HR3 on HR 1099)}  \\ \hline 
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$1.82^{+0.69}_{-0.62}$ / $21.1^{+8.0}_{-7.2}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $1.64^{+0.78}_{-0.37}$ /  $19.1^{+9.1}_{-4.3}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.11^{+0.16}_{-0.06}$} &                                   & $Z$ ($Z_{\odot}$) & $0.1^{+0.1}_{-0.09}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.11^{+0.29}_{-0.06}$} &                                   & $K^{\mathrm{apec}}$ & $0.14^{+0.19}_{-0.09}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.48^{+0.11}_{-0.08}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $0.20^{+0.14}_{-0.13}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{35 (26)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 29 (24) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.12} & \multicolumn{2}{c}{Null hyp. prob.} &   0.23  \\ \hline 
\end{tabular}
\end{center}
\label{tab:1114010127_block_all}
\end{table*}


==> table/HR1099/1114010128_block2.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:HR1099_HR4}b \& c.}
\begin{center}
\begin{tabular}{cccccc}
\hline 
\multicolumn{6}{c}{1114010128 GTI 2 (During Flare HR4 on HR 1099)}  \\ \hline 
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$2.57^{+0.85}_{-0.5}$ / $29.8^{+9.8}_{-5.8}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $2.57^{+0.42}_{-0.54}$ /  $29.8^{+4.9}_{-6.2}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.13^{+0.05}_{-0.05}$} &                                   & $Z$ ($Z_{\odot}$) & $0.13^{+0.05}_{-0.05}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.33^{+0.19}_{-0.13}$} &                                   & $K^{\mathrm{apec}}$ & $0.33^{+0.22}_{-0.12}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.49^{+0.11}_{-0.12}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $0.69^{+0.68}_{-0.65}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{23 (30)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 20 (28) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.8} & \multicolumn{2}{c}{Null hyp. prob.} &   0.85  \\ \hline 
\end{tabular}
\end{center}
\label{tab:1114010128_block2}
\end{table*}


==> table/HR1099/1114010128_block6.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:HR1099_HR4}d \& e.}
\begin{center}
\begin{tabular}{cccccc}
\hline 
\multicolumn{6}{c}{1114010128 GTI 6 (During Flare HR4 on HR 1099)}  \\ \hline 
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$2.68^{+0.99}_{-0.67}$ / $31.1^{+11.4}_{-7.8}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $2.44^{+1.08}_{-0.48}$ /  $28.3^{+12.6}_{-5.5}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.14^{+0.06}_{-0.06}$} &                                   & $Z$ ($Z_{\odot}$) & $0.13^{+0.06}_{-0.06}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.26^{+0.22}_{-0.1}$} &                                   & $K^{\mathrm{apec}}$ & $0.3^{+0.19}_{-0.14}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.48^{+0.08}_{-0.09}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $0.83^{+0.66}_{-0.61}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{33 (29)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 28 (27) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.28} & \multicolumn{2}{c}{Null hyp. prob.} &   0.4  \\ \hline 
\end{tabular}
\end{center}
\label{tab:1114010128_block6}
\end{table*}


==> table/HR1099/1114010133_block1.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:HR1099_HR5}b \& c.}
\begin{center}
\begin{tabular}{cccccc}
\hline 
\multicolumn{6}{c}{1114010133 GTI 1 (During Flare HR5 on HR 1099)}  \\ \hline 
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$5.44^{+1.4}_{-0.69}$ / $63.1^{+16.3}_{-8.1}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $5.35^{+1.26}_{-0.83}$ /  $62.1^{+14.7}_{-9.6}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.15^{+0.05}_{-0.04}$} &                                   & $Z$ ($Z_{\odot}$) & $0.15^{+0.05}_{-0.04}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.44^{+0.06}_{-0.08}$} &                                   & $K^{\mathrm{apec}}$ & $0.44^{+0.08}_{-0.07}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.42^{+0.06}_{-0.06}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $1.99^{+1.27}_{-1.26}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{45 (39)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 38 (37) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.23} & \multicolumn{2}{c}{Null hyp. prob.} &   0.4  \\ \hline 
\end{tabular}
\end{center}
\label{tab:1114010133_block1}
\end{table*}


==> table/HR1099/1114010133_block11.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:HR1099_HR5}f \& g.}
\begin{center}
\begin{tabular}{cccccc}
\hline 
\multicolumn{6}{c}{1114010133 GTI 11 (During Flare HR5 on HR 1099)}  \\ \hline 
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$2.96^{+0.82}_{-0.41}$ / $34.3^{+9.5}_{-4.8}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $2.91^{+0.77}_{-0.42}$ /  $33.7^{+8.9}_{-4.8}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.12^{+0.04}_{-0.03}$} &                                   & $Z$ ($Z_{\odot}$) & $0.11^{+0.04}_{-0.03}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.55^{+0.18}_{-0.17}$} &                                   & $K^{\mathrm{apec}}$ & $0.57^{+0.19}_{-0.17}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.5^{+0.07}_{-0.06}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $1.21^{+0.95}_{-0.96}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{47 (43)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 42 (41) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.33} & \multicolumn{2}{c}{Null hyp. prob.} &   0.42  \\ \hline 
\end{tabular}
\end{center}
\label{tab:1114010133_block11}
\end{table*}


==> table/HR1099/1114010133_block6.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:HR1099_HR5}d \& e.}
\begin{center}
\begin{tabular}{cccccc}
\hline 
\multicolumn{6}{c}{1114010133 GTI 6 (During Flare HR5 on HR 1099)}  \\ \hline 
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$4.08^{+1.07}_{-0.48}$ / $47.3^{+12.4}_{-5.5}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $4.1^{+1.17}_{-0.56}$ /  $47.5^{+13.6}_{-6.5}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.16^{+0.04}_{-0.04}$} &                                   & $Z$ ($Z_{\odot}$) & $0.14^{+0.04}_{-0.05}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.79^{+0.14}_{-0.18}$} &                                   & $K^{\mathrm{apec}}$ & $0.78^{+0.17}_{-0.18}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.54^{+0.04}_{-0.04}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $4.95^{+2.48}_{-2.33}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{55 (44)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 43 (42) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.12} & \multicolumn{2}{c}{Null hyp. prob.} &   0.43  \\ \hline 
\end{tabular}
\end{center}
\label{tab:1114010133_block6}
\end{table*}


==> table/HR1099/1114010136_block2.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:HR1099_HR6}b \& c.}
\begin{center}
\begin{tabular}{cccccc}
\hline 
\multicolumn{6}{c}{1114010136 GTI 2 (During Flare HR6 on HR 1099)}  \\ \hline 
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$3.08^{+0.89}_{-0.46}$ / $35.7^{+10.3}_{-5.4}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $2.89^{+0.8}_{-0.44}$ /  $33.5^{+9.3}_{-5.1}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.13^{+0.04}_{-0.04}$} &                                   & $Z$ ($Z_{\odot}$) & $0.13^{+0.04}_{-0.04}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.28^{+0.09}_{-0.09}$} &                                   & $K^{\mathrm{apec}}$ & $0.31^{+0.11}_{-0.1}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.37^{+0.04}_{-0.04}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $0.95^{+0.55}_{-0.55}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{68 (43)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 60 (41) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.01} & \multicolumn{2}{c}{Null hyp. prob.} &   0.03  \\ \hline 
\end{tabular}
\end{center}
\label{tab:1114010136_block2}
\end{table*}


==> table/HR1099/1114010153_block23.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:HR1099_HR7}b \& c.}
\begin{center}
\begin{tabular}{cccccc}
\hline 
\multicolumn{6}{c}{1114010153 GTI 2$+$3 (During Flare HR7 on HR 1099)}  \\ \hline 
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$5.94^{+0.61}_{-0.53}$ / $68.9^{+7.1}_{-6.1}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $5.91^{+0.54}_{-0.53}$ /  $68.5^{+6.3}_{-6.1}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.29^{+0.05}_{-0.04}$} &                                   & $Z$ ($Z_{\odot}$) & $0.3^{+0.04}_{-0.04}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.59^{+0.05}_{-0.05}$} &                                   & $K^{\mathrm{apec}}$ & $0.58^{+0.05}_{-0.04}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.38^{+0.03}_{-0.04}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $2.27^{+1.18}_{-1.19}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{65 (52)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 55 (50) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.11} & \multicolumn{2}{c}{Null hyp. prob.} &   0.3  \\ \hline 
\end{tabular}
\end{center}
\label{tab:1114010153_block23}
\end{table*}


==> table/Sigma_Gem/1200040104_block0.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:Sigma_Gem_S1}b \& c.}
\begin{center}
\begin{tabular}{cccccc}
\hline
\multicolumn{6}{c}{1200040104 GTI 0 (During Flare S1 on $\sigma$ Gem)}  \\ \hline
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$6.03^{+0.73}_{-0.78}$ / $70.0^{+8.4}_{-9.1}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $6.29^{+0.83}_{-0.86}$ /  $73.0^{+9.6}_{-10.0}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.16^{+0.04}_{-0.03}$} &                                   & $Z$ ($Z_{\odot}$) & $0.16^{+0.04}_{-0.03}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.51^{+0.07}_{-0.04}$} &                                   & $K^{\mathrm{apec}}$ & $0.51^{+0.06}_{-0.04}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.38^{+0.03}_{-0.04}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $-1.99^{+0.88}_{-0.86}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{74 (72)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 60 (70) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.43} & \multicolumn{2}{c}{Null hyp. prob.} &   0.81  \\ \hline
\end{tabular}
\end{center}
\label{tab:1200040104_block0}
\end{table*}


==> table/Sigma_Gem/1200040104_block5.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:Sigma_Gem_S1}d \& e.}
\begin{center}
\begin{tabular}{cccccc}
\hline
\multicolumn{6}{c}{1200040104 GTI 5 (During Flare S1 on $\sigma$ Gem)}  \\ \hline
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$3.11^{+1.27}_{-0.77}$ / $36.1^{+14.7}_{-8.9}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $2.99^{+1.12}_{-0.78}$ /  $34.7^{+13.0}_{-9.1}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.11^{+0.05}_{-0.05}$} &                                   & $Z$ ($Z_{\odot}$) & $0.11^{+0.05}_{-0.05}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.63^{+0.44}_{-0.24}$} &                                   & $K^{\mathrm{apec}}$ & $0.66^{+0.53}_{-0.24}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.45^{+0.1}_{-0.1}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $1.95^{+1.78}_{1.74}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{27 (29)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 23 (27) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.59} & \multicolumn{2}{c}{Null hyp. prob.} &   0.67  \\ \hline
\end{tabular}
\end{center}
\label{tab:1200040104_block5}
\end{table*}


==> table/Sigma_Gem/1200040106_block_all.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:Sigma_Gem_S1}f \& g.}
\begin{center}
\begin{tabular}{cccccc}
\hline
\multicolumn{6}{c}{1200040106 All (During Flare S1 on $\sigma$ Gem)}  \\ \hline
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$3.34^{+0.4}_{-0.53}$ / $38.7^{+4.6}_{-6.1}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $3.11^{+0.56}_{-0.38}$ /  $36.1^{+6.5}_{-4.4}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.08^{+0.02}_{-0.02}$} &                                   & $Z$ ($Z_{\odot}$) & $0.08^{+0.02}_{-0.02}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.22^{+0.07}_{-0.03}$} &                                   & $K^{\mathrm{apec}}$ & $0.24^{+0.06}_{-0.05}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.5^{+0.05}_{-0.07}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $0.36^{+0.28}_{0.27}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{85 (73)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 81 (71) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.16} & \multicolumn{2}{c}{Null hyp. prob.} &   0.20  \\ \hline
\end{tabular}
\end{center}
\label{tab:1200040106_block_all}
\end{table*}


==> table/UX_Ari/1100380101_block0.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:UX_Ari_U1}b \& c.}
\begin{center}
\begin{tabular}{cccccc}
\hline 
\multicolumn{6}{c}{1100380101 GTI 0 (During Flare U1 on UX Ari)}  \\ \hline 
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$4.93^{+4.32}_{-2.14}$ / $57.2^{+50.2}_{-24.8}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $4.08^{+4.29}_{-1.63}$ /  $47.3^{+49.7}_{-18.9}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.09^{+0.11}_{-0.09}$} &                                   & $Z$ ($Z_{\odot}$) & $0.08^{+0.09}_{-0.08}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.07^{+0.08}_{-0.03}$} &                                   & $K^{\mathrm{apec}}$ & $0.09^{+0.11}_{-0.04}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.48^{+0.07}_{-0.07}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $0.98^{+0.3}_{-0.58}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{45 (30)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 37 (28) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.04} & \multicolumn{2}{c}{Null hyp. prob.} &   0.12  \\ \hline 
\end{tabular}
\end{center}
\label{tab:1100380101_block0}
\end{table*}


==> table/UX_Ari/1100380106_block_all.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:UX_Ari_U2}b \& c.}
\begin{center}
\begin{tabular}{cccccc}
\hline
\multicolumn{6}{c}{1100380106 All (During Flare U2 on UX Ari)}  \\ \hline 
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$5.43^{+0.76}_{-0.77}$ / $63.0^{+8.8}_{-8.9}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $5.42^{+0.9}_{-0.87}$ /  $62.9^{+10.4}_{-10.1}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.16^{+0.04}_{-0.03}$} &                                   & $Z$ ($Z_{\odot}$) & $0.15^{+0.02}_{-0.03}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.36^{+0.06}_{-0.04}$} &                                   & $K^{\mathrm{apec}}$ & $0.36^{+0.07}_{-0.04}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.52^{+0.05}_{-0.04}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $1.36^{+0.9}_{-0.86}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{53 (55)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 46 (53) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.55} & \multicolumn{2}{c}{Null hyp. prob.} &   0.73  \\ \hline 
\end{tabular}
\end{center}
\label{tab:1100380106_block_all}
\end{table*}


==> table/UX_Ari/1100380109_block_all.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:UX_Ari_U4}b \& c.}
\begin{center}
\begin{tabular}{cccccc}
\hline
\multicolumn{6}{c}{1100380109 All (During Flare U4 on UX Ari)}  \\ \hline
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$4.78^{+1.29}_{-1.44}$ / $55.4^{+15.0}_{-16.7}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $4.6^{+1.38}_{-1.38}$ /  $53.3^{+16.1}_{-16.1}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.12^{+0.07}_{-0.06}$} &                                   & $Z$ ($Z_{\odot}$) & $0.12^{+0.07}_{-0.12}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.13^{+0.07}_{-0.03}$} &                                   & $K^{\mathrm{apec}}$ & $0.13^{+0.08}_{-0.03}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.48^{+0.21}_{-0.42}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $0.68^{+0.6}_{-0.59}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{34 (37)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 30 (35) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.61} & \multicolumn{2}{c}{Null hyp. prob.} &   0.69  \\ \hline
\end{tabular}
\end{center}
\label{tab:1100380109_block_all}
\end{table*}


==> table/UX_Ari/1100380113_block_all.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:UX_Ari_U4}d \& e.}
\begin{center}
\begin{tabular}{cccccc}
\hline
\multicolumn{6}{c}{1100380113 All (During Flare U4 on UX Ari)}  \\ \hline
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$1.33^{+0.33}_{-0.29}$ / $15.4^{+3.8}_{-3.3}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $1.31^{+0.3}_{-0.26}$ /  $15.2^{+3.5}_{-3.0}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.11^{+0.22}_{-0.07}$} &                                   & $Z$ ($Z_{\odot}$) & $0.1^{+0.16}_{-0.07}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.34^{+0.48}_{-0.18}$} &                                   & $K^{\mathrm{apec}}$ & $0.44^{+0.36}_{-0.27}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.44^{+0.07}_{-0.08}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $0.18^{+0.15}_{-0.15}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{54 (39)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 51 (37) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.05} & \multicolumn{2}{c}{Null hyp. prob.} &   0.07  \\ \hline
\end{tabular}
\end{center}
\label{tab:1100380113_block_all}
\end{table*}


==> table/UX_Ari/1100380118_block_all.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:UX_Ari_U4}f \& g.}
\begin{center}
\begin{tabular}{cccccc}
\hline
\multicolumn{6}{c}{1100380118 All (During Flare U4 on UX Ari)}  \\ \hline
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$1.08^{+0.08}_{-0.08}$ / $12.5^{+1.0}_{-1.0}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $1.08^{+0.09}_{-0.09}$ /  $12.5^{+1.1}_{-1.0}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$1.0$ (fix)} &                                   & $Z$ ($Z_{\odot}$) & $1.0$ (fix) \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.26^{+0.12}_{-0.08}$} &                                   & $K^{\mathrm{apec}}$ & $0.25^{+0.13}_{-0.08}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.35^{+0.06}_{-0.09}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $0.29^{+0.17}_{0.17}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{37 (17)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 29 (15) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.004} & \multicolumn{2}{c}{Null hyp. prob.} &   0.02  \\ \hline
\end{tabular}
\end{center}
\label{tab:1100380118_block_all}
\end{table*}


==> table/UX_Ari/1100380127_block34.tex <==
\begin{table*}
\caption{Best-fit spectral parameters of \texttt{apec} and \texttt{apec+gauss} models shown in Figure \ref{fig:UX_Ari_U5}b \& c.}
\begin{center}
\begin{tabular}{cccccc}
\hline
\multicolumn{6}{c}{1100380127 GTI 3$+$4 (During Flare U5 on UX Ari)}  \\ \hline
\multicolumn{3}{c|}{Without the additional Gaussiann}  & \multicolumn{3}{c}{With the additional Gaussiann} \\ \hline
\multirow{4}{*}{\texttt{apec}}                          & $kT$ (keV) / $T$ (MK)        & \multicolumn{1}{c|}{$2.58^{+4.19}_{-1.32}$ / $29.9^{+48.6}_{-15.3}$} & \multirow{4}{*}{\texttt{apec}}    & $kT$ (keV) / $T$ (MK)        & $2.6^{+6.24}_{-1.23}$ /  $30.1^{+72.4}_{-14.3}$   \\
                                                        & $Z$ ($Z_{\odot}$) & \multicolumn{1}{c|}{$0.17^{+0.22}_{-0.11}$} &                                   & $Z$ ($Z_{\odot}$) & $0.12^{+0.18}_{-0.12}$ \\
                                                        & $v \: (\mathrm{km \: s^{-1}})$               & \multicolumn{1}{c|}{$0.00$ (fix)} &                                   & $v \: (\mathrm{km \: s^{-1}})$ & $0.00$ (fix)   \\
                                                        & $K^{\mathrm{apec}}$              & \multicolumn{1}{c|}{$0.12^{+0.63}_{-0.12}$} &                                   & $K^{\mathrm{apec}}$ & $0.09^{+0.48}_{-0.06}$    \\ \cline{4-6}
\multirow{3}{*}{---}                          & --- & --- & \multirow{3}{*}{\texttt{gauss}}    & $E_{l}$ (keV) &   $6.55^{+0.11}_{-0.19}$ \\
                                                    & --- & --- &                                  & $\sigma$(keV) &   $0.00$ (fix)  \\
                                                    & --- & ---  &                       & $K^{\mathrm{gauss}}$ &  $0.73^{+0.83}_{-0.65}$  \\ \hline
\multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)}                                     & \multicolumn{1}{c|}{17 (21)} & \multicolumn{2}{c}{$\chi^{2}$ (d.o.f.)} & 14 (19) \\
\multicolumn{2}{c}{Null hyp. prob.} & \multicolumn{1}{c|}{0.69} & \multicolumn{2}{c}{Null hyp. prob.} &   0.79  \\ \hline
\end{tabular}
\end{center}
\label{tab:1100380127_block34}
\end{table*}

